Active Safety Envelopes using Light Curtains with Probabilistic Guarantees

To safely navigate unknown environments, robots must accurately perceive dynamic obstacles. Instead of directly measuring the scene depth with a LiDAR sensor, we explore the use of a much cheaper and higher resolution sensor: programmable light curtains. Light curtains are controllable depth sensors that sense only along a surface that a user selects. We use light curtains to estimate the safety envelope of a scene: a hypothetical surface that separates the robot from all obstacles. We show that generating light curtains that sense random locations (from a particular distribution) can quickly discover the safety envelope for scenes with unknown objects. Importantly, we produce theoretical safety guarantees on the probability of detecting an obstacle using random curtains. We combine random curtains with a machine learning based model that forecasts and tracks the motion of the safety envelope efficiently. Our method accurately estimates safety envelopes while providing probabilistic safety guarantees that can be used to certify the efficacy of a robot perception system to detect and avoid dynamic obstacles. We evaluate our approach in a simulated urban driving environment and a real-world environment with moving pedestrians using a light curtain device and show that we can estimate safety envelopes efficiently and effectively. Project website: https://siddancha.github.io/projects/active-safety-envelopes-with-guarantees

==> misc/intro-notes.tex <==
\section{Notes for introduction}

\subsection{Parah 1: Environment and challenges}
\begin{enumerate}
    \item Consider a robot navigating in an unknown enviroment. The environment may contain objects that are arbitrarily distributed, whose motion is haphazard and unpredictable, and that may enter and leave the environment in an undetermined manner. This situation is commonplace in a variety of robotics tasks such as automous driving, indoor and outdoor robot navigation, mobile robotics, robot delivery etc. How do we ensure that the robot moves safely in the environment and avoids collision with obstacles whose locations are apriori unknown?
\end{enumerate}

\subsection{Parah 2: Define safety envelope}
\begin{enumerate}
    \item Many tasks in robotics require safety guarantees.
    \item Define what a safety envelope is.
    \item Subtle difference between 2D and 3D depth.
\end{enumerate}

\subsection{Parah 3: Introduce light curtains}
\begin{enumerate}
    \item One approach to find safety envelopes is to first predict the full depth map of the environment. Then, the result can be post-processed to compute the safety envelope.
    \item Predicting or measuring the full depth map is the dominant paradigm in depth sensing and perception. However, this may be inefficient.
    \item Philosophy of active perception: no point in sensing the entire scene uniformly.
    \item Instead, we directly estimate the safety envelopes.
    \item Benefits of light curtains from ECCV paper.
    \item Adaptively place curtains in the environment.
    \item By directly predicting the safety envelope, we avoid both the complexity in predicting the full depth map, as well as the post-processing required to infer the envelope from the full depth.
    \item Provide theoretical guarantees of finding it.
    \item We will use the terms ``curtains'' and ``safety envelopes'' interchangeably.
    \item Dave's point that safety envelopes using light curtains are not sufficient for complete scene perception, and are not intended to be a replacement for sensors such as LiDARs, but they can be an important supplement for ensuring safety and obstacle avoidance in robot navigation.
\end{enumerate}

\subsection{Parah 4: Random curtains}
\begin{enumerate}
    \item We need to detect the safety envelope of objects whose locations are unknown, in order to avoid colliding with them.
    \item Previous work [Bartels] has shown that placing random curtain can quickly discover objects.
    \item In this work, we develop a systematic framework to generate random curtains that respect the physical constraints of the light curtain device.
    \item Importantly, we develop a method that provides theoretical guarantees on the probability of random curtains detecting objects in the environment and identifying the safety envelope.
\end{enumerate}

\subsection{Parah 5: Learning to track the safety envelope}
\begin{enumerate}
    \item Once a part of the safety envelope (such as an object surface) is discovered, it may be ineffecient and sometimes unnecessary to keep exploring the scene randomly. Instead, a more efficient strategy is to forecast how the safety envelope will move in the next timestep, and track it by sensing at that predicted location.
    \item Machine learning based methods could be trained to forecast and track the envelope. However, it is often hard to develop theoretical guarantees on the performance of machine learning models, especially neural networks.
    \item On the other hand, our method is able to provide probabilistic guarantees for safety envelope discovery by random curtains.    
\end{enumerate}

\subsection{Parah 6: Combining random curtains and learning}
\begin{enumerate}
    \item In this work, we leverage the best of both worlds. By combining deep neural networks with random light curtain placements, we are able to predict and track safety envelopes efficiently, while furnishing probabilistic guarantees for discovering them.
    \item Both of these are crucial components for accurately identifying the safety envelope of a scene, towards building a robot perception system that can safely and efficiently detect obstacles to avoid.
    \item Summarize our results.
\end{enumerate}

\subsection{Previous points that may still be useful}
\begin{enumerate}
    \item Any light curtain algorithm that accurately tracks scene depth must also intermittently explore the environment to find untracked objects. This is necessary for two reasons. First, the light curtain algorithm may lose track of objects from time to time (especially fast-moving objects) and will need to re-detect them. Second, new objects might appear in the scene that weren't previously being tracked.
    \item their efficacy can be evaluate and certified in a principled way. This can, for example, be used to provide safety guarantees on the ability of a robot perception system deployed in an autonomous driving vehicle to detect obstacles and avoid collisions.
\end{enumerate}
